Causal Distillation for Alleviating Performance Heterogeneity in Recommender Systems

Recommendation performance usually exhibits a long-tail distribution over users -- a small portion of head users enjoy much more accurate recommendation services than the others. We reveal two sources of this performance heterogeneity problem: the uneven distribution of historical interactions (a natural source); and the biased training of recommender models (a model source). As addressing this problem cannot sacrifice the overall performance, a wise choice is to eliminate the model bias while maintaining the natural heterogeneity. The key to debiased training lies in eliminating the effect of confounders that influence both the user's historical behaviors and the next behavior. The emerging causal recommendation methods achieve this by modeling the causal effect between user behaviors, however potentially neglect unobserved confounders (\eg, friend suggestions) that are hard to measure in practice. To address unobserved confounders, we resort to the front-door adjustment (FDA) in causal theory and propose a causal multi-teacher distillation framework (CausalD). FDA requires proper mediators in order to estimate the causal effects of historical behaviors on the next behavior. To achieve this, we equip CausalD with multiple heterogeneous recommendation models to model the mediator distribution. Then, the causal effect estimated by FDA is the expectation of recommendation prediction over the mediator distribution and the prior distribution of historical behaviors, which is technically achieved by multi-teacher ensemble. To pursue efficient inference, CausalD further distills multiple teachers into one student model to directly infer the causal effect for making recommendations.

==> sections/1.IntroductionOld.tex <==

\section{Introduction}


Recommender Systems alleviate the information overload on the Web by providing personalized services for users to seek information~\todo{cite}.
%for users by discovering information and content that users will interact with. As such, recommendation models exploit users' historical interactions, e.g., clicks, for training \todo{cite a lot}, aiming to accurately measure the correlation of each user-item pair. 
It has become a default choice to learn recommender model from historical user-item interactions by estimating the correlation between users and items~\cite{}. The model typically exhibits a performance heterogeneity with significant divergence across different user groups.
Figure~\ref{fig:longtail_base} provides an empirical evidence where 
%However, as shown in Figure \ref{fig:longtail_base}, we observe that recommendation performance is discrepant and even exhibits a long-tail distributions over users. Specifically,
we train a representative recommender model DIN~\todo{cite} recommender on the benchmark Amazon Review dataset and evaluate the performance over equally-sized user groups. We consider two factors to cluster users: 1) the activeness of user (\ie, the number of interactions for training); 2) and the users' behavior consistency on popular items\footnote{We cluster items into groups by their popularities. Then we split the behavior sequence of each user in the middle and transform both parts into item popularity distributions according to the clusters. We refer to the KL divergence of these two distributions as behavior consistency.}. The results show that a small portion of head users receive more accurate recommendation than the others. 
%To obtain a strustable recommendation in the long run, 
It is undoubtedly essential to alleviate the \textbf{performance heterogeneity} issue in recommender systems.


%--------------------------------fig---------------------
\begin{figure}[!t] \begin{center}
    \includegraphics[width=\columnwidth]{./figures/longtail_base.pdf}
    \caption{
    	TODO
	}
\label{fig:longtail_base}
\end{center} \end{figure}
%--------------------------------fig end---------------------




Obviously, there is a \textit{natural source} for performance heterogeneity. For example, users' interests on items are internally discrepant, leading to heterogenous behavior data distributions. Active users with more logged interactions on recommender systems are more likely to obtain a comprehensive interest modeling. The \textit{natural source} is inevitable, and explicitly regularizing the performance over users to be close might hurt the overall effectiveness, such as fairness-related methods \todo{cite}. However, in real-world recommender systems, there are various factors that cause spuriously correlated user-item interactions. For example, active users might appear to be more aimless, and thus clicking more items that are less related to their internal interests. Some users regard popular items as the ones of high quality, and thus producing behaviors highly correlated to items' popularities. We use Directed Acyclic Graphs (DAGs) borrowed from causality \todo{cite} for a better illustration, as shown in Figure \ref{fig:causalGraph}. The above mentioned factors (user activeness, and users behaviors on item popularities) are called confounders $Z$ in causality \todo{cite}, which are the common cause of users $X$ and items $Y$. Unfortunately, recommenders are easily affected by confounding effects $X \leftarrow Z \rightarrow Y$ when estimating the causal effect $X \rightarrow Y$ with observed data samples. Without intervention, the model might draw false conclusions about users and items, \eg, inaccurate click-through-rate predictions, plagued by spurious correlations. Worse still, as shown in Figure \ref{fig:longtail_base}, we found that long-tail users are more sensitive to confounding effects, and suffer from an enlarged performance heterogeneity problem, \ie, an \textit{artificial source} caused by spurious correlation \footnote{To be specific, we train one DIN models per user group. We observe that the recommendation performance when individually trained is better than the performance when jointly trained with other users' interactions.}. Therefore, it is urgent need to avoid the artificial source and alleviate the spurious correlation in prediction.



Recently, much research progress has been made in debiasing recommender training by embracing causal theory. According to their major requirements, methods that reduce confounding effects can be roughly categorized into two lines.  The first line of works assume the unconfoundedness \todo{cite}, which means all the confounders affecting both users and items are observed. However, the assumption might not hold in unconstrained real-world recommender systems, and there are always considerable confounders that are not observed by the model or even by the recommender system. For example, social (\eg, friends) recommendation that causes users and items to have interactions might not be captured by the recommender system. The second line of works can handle unobserved confounders by introducing unbiased data \todo{cite}. Unbiased data is collected under constrained environment. For example, uniform data is collected when items exposed to users are uniformly sampled. Obviously, these data samples are not routinely available and mostly expensive to collect since constrained environment might hurt users' experiences. Therefore, it is in urgent need for a method to deal with various and even unobserved confounders without costly unbiased data.



%Many of them deal with popularity bias \todo{cite}, and exposure bias \todo{cite}, via uniform data \todo{cite}, inverse propensity score (IPS) \todo{cite}, and disentanglement \todo{cite}. 


%Most of them investigate a certain kind of bias, which is often observed by the model. Unfortunately, in real-world recommender systems, the confounders that cause performance heterogeneity can be various -- not limited to the user activeness. For example, popular items are more likely to appear in the front-page or occupy a large portion of the page. Therefore, in the data production process, item popularity can lead to co-occurrence of user-items, disregarding users' internal interests, \ie, the confounding effects.



%We reveal two sources of performance heterogeneity. 
%First of all, users' interests on items are internally discrepant
%
%the behavior data distribution over users are by nature not independent and identically distributed, due to users' discrepant interests on items.  We summarize it as the \textit{natural source}
%
%factors that diversify users' data distributions are far beyond users' internal preferences on items. For example, active users might appear to be more aimless, and thus clicking more items that are less related to their internal interests. Some users regard popular items as the ones of high quality, and thus producing behaviors highly correlated to items' popularities.





%The heterogeneity of users' behavior data distribution poses challenges for model training. Recommendation models are found to be easily biased towards some privileged users \todo{cite a few}, e.g., users having more interactions logged, or users that consistently clicks popular items. As a result, as shown in Figure \ref{fig:causalGraph}, the performance of different users renders a long-tail distribution -- most users suffer from low-quality recommendations. We take an in-depth analysis on inactive users. For the last 20\% users who have the fewest data samples for training, the NDCG@10 becomes $0.4732 \rightarrow TODO / 0.4747 \rightarrow TODO$ when training each 10\% using a separate model.
%% when we train separated models for the last two long-tail inactive user groups on Amazon dataset, the NDCG@10 are TODO/TODO compared to NDCG@10 $0.4732/0.4747$ of the model that is trained on all data samples. 
% In other words, the model training enlarge the Matthew Effect. Due to the feedback loop of recommender systems, ignoring this performance heterogeneity problem might result in a less satisfied platform ecosystem.
%
%%Unfortunately, few works in the literature investigate the underlying cause of the \textbf{\textit{performance heterogeneity}} of different users. Since causality has been widely used in regularizing model training, we analyze the 
%Unfortunately few works in the literature investigate the underlying cause of the \textbf{\textit{performance heterogeneity}} of different users. We take the initiative and propose to analyze the problem using causality and directed acyclic graphs (DAGs), as shown in Figure \ref{fig:causalGraph}.
%For recommender systems, inferior performance comes from the inferior assessment of the true correlation of users $X$ and items $Y$, i.e., the causal effects $X \rightarrow Y$. In light of this, during training/prediction, the model captures some spurious correlations $X \leftarrow Z \rightarrow Y$ among users and items, while the severity levels of spurious correlations for different users are heterogeneous. For example, 
%%in recommender systems, users' activeness typically renders a long-tail distribution,
%% -- a small portion of active users have the majority of interactions logged
%%as shown in Figure \ref{fig:causalGraph}. 
%%It is safe to suppose that there are some recommendation patterns that can be shared among similar users, i.e., collaborative filtering, no matter these users are active or not. However, 
%in average, active users might be more aimless and thus producing many user-item pairs with weak correlations.
%%In the data production process, active users will click many positive items they like and also many false-positive items they eventually dislike. 
%From the causal view, the activeness $Z$ becomes the confounder of users and items, leading to spurious correlations that are beyond the true causal effects. 
%%With the confounder, recommendation models will be easily misled in measuring the correlation of user-item pairs. 
%Obviously, inactive users suffer more from the negative effect of activeness -- the severity levels of the spurious correlation caused by users' activeness differ from users to users.
%
%
%%Therefore, popularity bias becomes the confounder of both users and items. 
%The severity level of the spurious correlation caused are heterogeneous among users. For example, the total effect can be approximately equal to the causal effect for users that regard popular items as high-quality ones and prefer to click them. What makes the performance heterogeneity more severe is that many of the confounders are even unobserved to the model. For example, the production of user-item pairs might be affected by the recommendation of friends, which is unseen to the model. Therefore, how to handle multiple confounders and unobserved confounding effects is an important challenge but remains largely unexplored in the literature.



%--------------------------------fig---------------------
\begin{figure}[!t] \begin{center}
    \includegraphics[width=\columnwidth]{./figures/Confouding.pdf}
    \caption{
    	Causal graph for illustrating a) the enlarged performance heterogeneity due to confounding effects; and b) two-stage modeling procedure of front-door adjustment.
	}
\label{fig:causalGraph}
\end{center} \end{figure}
%--------------------------------fig end---------------------





To address the aforementioned challenges, we propose to adopt a causal inference technique, \ie, front-door adjustment, inspired by the literature of social sciences \todo{cite a few}. Different from many other techniques, such as back-door adjustment, front-door adjustment dose not assume unfoundedness, and can hereby alleviate various confounding effects that are even unobserved to the model. As shown in Figure \ref{fig:causalGraph}, front-door introduces a mediator and expands the causal graph. Then, front-door adjustment takes a two-stage modeling procedure: 1) estimating the causal effect $X \rightarrow M$ by modeling the mediator distribution, which requires heterogeneous sampling on the mediator $M$ given the treatment $X$; and 2) estimating the causal effects $M \rightarrow Y$ using do-calculus, \ie, $P(Y|do(M))$. 
However, there are two dilemmas in performing front-door adjustment on recommender systems. The first challenge comes from the heterogeneous and counterfactual sampling of $M$ given $X$. A deterministic recommender can hardly satisfy the condition. Another challenge relates to the expensive expectation computation on the outcome $Y$ over the distribution of both $M$ and $X$, \wrt the strict inference/serving latency restrictions in recommender systems.
To tackle these challenges, we encapsulate multi-teacher distillation into the instantiation of front-door adjustment, and propose the causal distillation framework, named \textbf{\textit{CausalD}}. CausalD employs the pre-trained heterogeneous teachers to perform counterfactual sampling of $M$ give $X$, and thus addressing the first challenge. Essentially, CausalD distills causal effects from heterogenous teachers, and guide the student to make predictions that are free from unobserved confounding effects. Therefore, the model used for inference/serving remains the same the oracle, and addresses the second challenge. In summary, this work makes the following key contributions:
\begin{itemize}[leftmargin=*]
	\item We analyze how model training enlarges the performance heterogeneity problem in recommender systems with causal graph; we identify that the bad impact stems from the confounding effects caused by various and even unobserved confounders.
	\item We propose a \textit{causal multi-teacher distillation} (CausalD), a novel framework that causally intervene model inference by distilling causal effects from heterogenous teachers.
	\item We instantiate CausalD on two base models (DIN and DeepFM), and conduct extensive experiments on three real-world datasets, validating the effectiveness of our causal analysis and CausalD.
\end{itemize}


%\clearpage


\iffalse

Bias in recommendation system





写作参考文献：
Deconfounded Recommendation for Alleviating Bias Amplification

Graph Prototypical Networks for Few-shot Learning on Attributed Networks




\fi









\iffalse





思路一：Distillation 存在 bias 问题，我们提出了一种 因果debias方法 缓解了Distillation中存在的bias问题，并应用到推荐上：
	问题1:为什么
思路二：推荐系统中存在bias问题，我们提出了一种因果debias方法，利用多teacher ensemble 蒸馏 + 前门/后门 调整 



【老idea】

Distillation

是直接讲Distillation 还是讲小一点 Distillation for recommender system



? Bias Amplification
	如果讲Bias Amplification，是否要做一些可视化或小实验？


	

? Confounding 效应
	confounding 和 bias amplification的关系？
	
	
？ 三种效应： Causal Effects; Confounding Effect; Endougenous Selection Bias
	作用：引出Confounding effects，从而讲我们如何解决confounding effects
	
	
%？ 讲出解决confounding bias的两种常用（在social science中可能是最常用的）的方法，backdoor和frontdoor


我们提出了Debiased Distillation from Biased Teachers 框架，结合使用了front-door adjustment 和 back-door adjustment两种常用（在social science中可能是最常用的）的方法，分别解决了蒸馏框架中的unobserved 和 observed confounder的问题。具体而言：
？ Front-door Adjustment
	优点：能够解决 unobserved confounding 的问题
	应用上的挑战，需要引入mediator，并对 Mediator 进行合理的采样；在蒸馏框架中，可以自然的使用teacher来实现给定X对M的采样（采样似乎就涉及多多个teacher了，有点没讲清楚），然而，teacher的采样会引入confounding bias，因为这种效应因此我们使用backdoor对teacher在mediator采样过程中引入的confounding效应进行了消除。
	？有些难讲，分组策略是否应当放在intro里面说，感觉是需要的，不然biased teachers从何而来
		我们对数据进行了主动分类讨论，并依次训练出了多个biased teachers，每个teacher相当于在某种特定取值confounder=z下训练得到的模型。因此是 P(Y|X, Z=z)






\fi



















